Trajectory Inference with Smooth Schr\"odinger Bridges

Motivated by applications in trajectory inference and particle tracking, we introduce Smooth Schr\"odinger Bridges. Our proposal generalizes prior work by allowing the reference process in the Schr\"odinger Bridge problem to be a smooth Gaussian process, leading to more regular and interpretable trajectories in applications. Though na\"ively smoothing the reference process leads to a computationally intractable problem, we identify a class of processes (including the Mat\'ern processes) for which the resulting Smooth Schr\"odinger Bridge problem can be lifted to a simpler problem on phase space, which can be solved in polynomial time. We develop a practical approximation of this algorithm that outperforms existing methods on numerous simulated and real single-cell RNAseq datasets. The code can be found at https://github.com/WanliHongC/Smooth_SB

==> content.tex <==
\begin{abstract}
Motivated by applications in trajectory inference and particle tracking, we introduce \emph{Smooth Schrödinger Bridges}. Our proposal generalizes prior work by allowing the reference process in the Schrödinger Bridge problem to be a smooth Gaussian process, leading to more regular and interpretable trajectories in applications. Though naïvely smoothing the reference process leads to a computationally intractable problem, we identify a class of processes (including the Matérn processes) for which the resulting Smooth Schrödinger Bridge problem can be \textit{lifted} a simpler problem on phase space, which can be solved in polynomial time. We develop a practical approximation of this algorithm that outperforms existing methods on numerous simulated and real single-cell RNAseq datasets. 
\end{abstract}
\section{Introduction}
The \textit{trajectory inference problem}---reconstructing the paths of particles from snapshots of their evolution---is fundamental to modern data science, with applications in single-cell biology~\cite{HugMagTon22, SaeCanTod19, SchShuTab19, ShaQiuZho23, TonHuaWol20}, fluid dynamics~\cite{BruNoaKou20,OueXuBod06}, and astronomical object tracking~\cite{KubDenGra07,LioSmaSwe20}.
Given observations of a collection of indistinguishable particles at discrete times, the statistician aims to infer the continuous trajectories that generated this data.

A leading approach~\cite{CheConGeo19,ChiZhaHei22,LavZhaKim24} builds on \citeauthor{Sch31}'s remarkable thought experiment~\citep{Sch31,Sch32}, formulating trajectory inference as a Kullback--Leibler minimization problem.
Suppose that a set of particles is observed at times $t_0, \dots, t_K \in [0, 1]$ and that the particles' arrangement at time $t_k$ is represented by a probability measure $\mu_k$, for all $k \in [K]$.
The \textit{multi-marginal Schrödinger bridge} corresponding to these observations is the solution of
\begin{align}
	\min_{P \in \mathcal{P}(\Omega)} \mathrm{D}(P | R) \label{obj: full_schrodinger}
	\text{ s.t. } P_{k} =\mu_{k}, \, \, \forall k \in [K],
\end{align}
where $D$ is the Kullback--Leibler divergence, $P_k$ denotes the time marginal of $P$ at time $t_k$, and $R$ is the law of a reference process, typically Brownian motion. (See \cref{sec:notation} for a complete list of notation.)
This formulation has an elegant quasi-Bayesian interpretation: the Schrödinger bridge matches the observed marginal distributions while keeping particle trajectories as faithful as possible to the prior $R$.

While extensively studied both theoretically and methodologically, this classical Schrödinger Bridge (SB) approach has a critical limitation: its trajectories inherit the roughness of Brownian paths,
leading to noisier estimators and less interpretable posterior paths; see Figure~\ref{FIG:Petal_f1}, left side.
Moreover, when the experimenter aims to track the positions of individual particles in a system evolving over time, inference with the Brownian motion prior fails to ``borrow strength'' from adjacent time points, resulting in less accurate results; see Figure~\ref{FIG:Matern_1D}, left side.

The literature on trajectory inference contains various proposals for encouraging smooth paths, inspired by spline algorithms on $\bR^d$ or the dynamics of physical systems.
(A full comparison with prior work appears in~\cref{sec:prior}.)
However, from the perspective of Schrödinger's original formulation, these modifications sacrifice the clear statistical interpretation of~\eqref{obj: full_schrodinger}.
We develop a new approach: a smooth version of the Schrödinger Bridge problem in which the Brownian motion is replaced by a smooth Gaussian process.
This proposal has an appealing statistical grounding: like Gaussian process regression~\cite{RasWil06}, it provides a flexible and principled way to perform non-parametric estimation while incorporating prior smoothness assumptions.
As Figures~\ref{FIG:Petal_f1} and~\ref{FIG:Matern_1D}, right side, show, the resulting estimates significantly outperform the vanilla Schrödinger Bridge, producing better estimates with smoother paths.

\textbf{Our contributions:} \\
\begin{itemize}
	\item We propose a class of Gaussian processes suitable as priors for smooth SB problems, which we show can be \textit{lifted} to simpler SB problems on phase space.
	\item We show that a message passing algorithm for the resulting lifted SB problem converges in time quadratic in $K$, an exponential improvement over the baseline approach.
	\item We develop an efficient approximation of our algorithm that outperforms existing methods in practice, in several cases by 2--5x.
\end{itemize}

\section{Prior work}\label{sec:prior}
There has been significant prior work on both the Schrödinger bridge problem and its applications in trajectory inference.
Here, we briefly survey some important related contributions.

The Schrödinger bridge has been the subject of significant theoretical interest since its introduction; see~\cite{Leo14} for historical details and additional context.
Currently, there are many methodological approaches to the Schrödinger bridge problem~\citep[see, e.g.][]{De-ThoHen21,GusKolKor23,PavTriTab21,PooNil24}, almost all of which focus on the two-marginal case (in our notation $K = 1$).
As was forcefully pointed out by~\citeauthor{AltBoi22}, the multi-marginal case presents significantly greater computational challenges~\citep{AltBoi22, AltBoi23}; indeed, no general-purpose algorithms with running time polynomial in $K$ exist.
However, it is possible to obtain polynomial-time algorithms in certain special cases~\cite{AltBoi23}.
Our work shows that smooth Schrödinger bridges with GAP priors are such a case.

The connection between multi-marginal entropic OT problems and belief propagation has been highlighted in a number of prior works dating back more than two decades~\cite{SinZhaChe22,TehWel01}, though apparently without connection to smooth Schrödinger Bridge problems.
The exception is the ``momentum Schrödinger bridge'' of~\citep*{CheConGeo19,CheLiuTao23}, which is, implicitly, an example of a smooth Schrödinger with prior given by integrated Brownian motion; the Sinkhorn algorithm proposed in~\cite{CheConGeo19} can be viewed as an \textit{ad hoc} version of belief propagation for this special case.
However, those works do not make the connection with smooth Gaussian processes, and their algorithm does not apply to more general GAPs.

The importance of the Schrödinger bridge problem for trajectory inference was implicitly recognized in the pioneering work~\cite{SchShuTab19}, and developed mathematically by~\cite{ChiZhaHei22,LavZhaKim24}.
The fact that the vanilla Shrödinger bridge problem uses a Markov prior is crucial for algorithms~\cite{ChiZhaHei22}, but has also been recognized as an undesirable feature that has led to the development of different trajectory inference methods which give rise to smoother paths.
Apart from~\cite{SheBerBro24}, which proposes a ``robust'' version of the Schrödinger Bridge problem in which a single reference process is replaced by a family of (Markov) reference processes, these alternate methods largely abandon Schrödinger's formulation and develop very different techniques.
Many of the most successful methods are based on measure-valued generalizations of splines~\cite{banerjee2024efficient,BenGalVia19, CheConGeo18,pmlr-v130-chewi21a,clancy2022wasserstein,JusRumErb24}.
Other methods based on neural networks have also been proposed~\cite{HugMagTon22,TonHuaWol20}.
We compare these methods in our experimental section.


\section{Background}\label{sec:background}
\subsection{The Multi-Marginal Schrödinger Bridge}
Let $R$ be a measure on the space $\Omega = C([0, 1]; \mathbb{R}^d)$ of continuous $\mathbb{R}^d$-valued paths, and let $\mu_0, \dots, \mu_K$ be probability measures on $\mathbb{R}^d$.
Fix a sequence of times $t_0 = 0 < t_1 \cdots < t_K = 1$.
Given $\omega \in \Omega$, we write $\omega_k = \omega(t_{k})$ for $k \in [K]$.
Given a probability measure $P$ on $\Omega$ and $k \in [K]$, let $P_k$ be the marginal distribution of $P$ at time $t_k$, that is, let $P_k$ be the element of $\mathcal{P}(\mathbb{R}^d)$ obtained by pushing $P$ forward under the map $\omega \mapsto \omega_k$.
The multi-marginal Schrödinger Bridge~\eqref{obj: full_schrodinger} exists under suitable moment conditions on $\mu_0, \dots, \mu_K$~\cite{Leo14}, and the strict convexity of the Kullback--Leibler divergence guarantees that when a solution exists, it is unique.

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{../Figures/icml_compare_Petal_f1.png}
	\caption{Comparison between the classical SB and smooth SB with Matérn prior on a trajectory inference task for the petal dataset~\cite{HugMagTon22}.  Colored points are observed data and paths are inferred trajectories. Our smooth SB approach generates much smoother and more concentrated trajectories.}
		\label{FIG:Petal_f1}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=.8\textwidth]{../Figures/icml_compare_Matern_f2.png}

	\caption{Comparison between the classical SB and smooth SB. The observations come from 20 independent trajectories of a Matérn Gaussian process with $\nu = 3.5$. The two pictures depict the posterior identification of particles obtained by solving the SB problem with two different priors. Our smooth SB approach recovers trajectories much more accurately.}
		\label{FIG:Matern_1D}
\end{figure}
Though phrased as a minimization problem over the space $\cP(\Omega)$, the Schrödinger bridge problem admits a ``static'' reformulation as a multi-marginal entropic optimal transport problem over the space $\cP(\bR^{d(K+1)})$.
Write $R_{[K]}$ for the joint law of $\bomega := (\omega_{0}, \dots, \omega_{K})$ for $\omega \sim R$.
\begin{lemma}\label{lem:dyn_to_stat}
	There is an one-to-one correspondence between solutions to~\eqref{obj: full_schrodinger} and solutions to
	\begin{equation}\label{eq:static_sb}
		\min_{P_{[K]} \in \cP(\bR^{d(K+1)})} \mathrm{D}(P_{[K]} | R_{[K]}),~~P_{k} =\mu_{k},~~\forall k \in [K].
	\end{equation}
	Moreover, if each measure $\mu_k$ is absolutely continuous with finite entropy and $R_{[K]}$ has density $\exp(- C(\bomega))$, then this problem is equivalent to
	\begin{equation}\label{eq:eot_problem}
		\min_{P_{[K]} \in \cP(\bR^{d(K+1)})} \int C(\bomega)  P_{[K]}{(\bomega)}\, d \bomega+ \mathrm{D}\left(P_{[K]} \Big| \bigotimes_{k = 0}^K \mu_k \right)~~P_{k} =\mu_{k},~~\forall k \in [K].
	\end{equation}
\end{lemma}
The reformulation in Lemma~\ref{lem:dyn_to_stat} is essential because it eliminates the need to optimize over probability measures on the infinite-dimensional space $\Omega$.
Though~\eqref{eq:eot_problem} was derived for absolutely continuous measures, the expression is sensible for arbitrary marginal measures.
We, therefore, take~\eqref{eq:eot_problem} as the basic definition of the multi-marginal Schrödinger bridge in what follows.
Importantly, when the measures $\mu_k$ are finitely supported, the resulting optimization problem is finite-dimensional.

\subsection{Sinkhorn's algorithm for multi-marginal transport}
Specializing to the case where each of the marginals $\mu_k$ is supported on a finite set $\cX_k$ of size at most $n$, the joint measure $P_{[K]}$ can be represented by a finite---albeit exponentially large---order $(K+1)$ tensor, of total size $n^{K+1}$.

A direct method to solve~\eqref{eq:eot_problem} in this case uses \citeauthor{Sin67}'s celebrated scaling Algorithm \ref{alg: Multi_Sinkhorn}.
Sinkhorn's algorithm is based on the observation that the optimal solution $P^*_{[T]}$ to~\eqref{eq:eot_problem} is of the form $P^*_{[T]}(\bx) = \exp(-C(\bx)) \prod_{k=0}^K v^*_k(x_k)$ for all $\bx = (x_0, \dots, x_K) \in \prod_{k=0}^K \cX_k$, for some ``scaling functions'' $v^*_k: \cX_k \to \bR^+$, $k \in [K]$.
\Cref{alg: Multi_Sinkhorn} produces a sequence of iterates $v^{(\ell)}_k$, $k \in [K]$, $\ell \geq 0$, which converge to these optimal scalings.


\begin{algorithm}
    \caption{Vanilla Sinkhorn Algorithm} \label{alg: Multi_Sinkhorn}
    
    \begin{algorithmic}
        \STATE \textbf{Input:} $\mu_0, ..., \mu_K$
        \STATE Initialize $v^{(0)}_0$, ..., $v^{(0)}_K \in ({\mathbb{R}^{+}})^n$, $\ell = 0$.
        \WHILE{not converged}
                \STATE $\ell \gets \ell + 1$
        \FOR{$k = 0, ..., K$}
        \STATE Compute $\mathbf{S}^{(\ell)}_k$ using  \eqref{eq: augmented_sinkhorn_calculate_marginal} with $\left\{ v^{(\ell)}_i\right\}_{i < k}$ and $\left\{ v^{(\ell-1)}_i\right\}_{i > k}$
        \STATE $v^{(\ell)}_k \leftarrow \mu_k \oslash \mathbf{S}^{(\ell)}_k$
        \ENDFOR
        \ENDWHILE
        \STATE Return $(v^{(\ell)}_k)_{k \in [K]}$
    \end{algorithmic}
\end{algorithm}


The key subroutine in \cref{alg: Multi_Sinkhorn} is an operation called ``marginalization'': given current iterates $(v_i)_{i \in [K]}$, the marginalization along coordinate $k$ is the function $\mathbf{S}_k: \cX_k \to \bR^+$ defined by
\begin{equation}
	\mathbf{S}_k(x_k) := \sum_{\substack{i = 0 \\ i \neq k}}^{K} \sum_{x_i \in \cX_i} \exp(-C(\bx)) \prod_{\substack{i = 0 \\ i \neq k }}^{K} v_i(x_i) \,. \label{eq: augmented_sinkhorn_calculate_marginal}
\end{equation}
The complexity of computing $\mathbf{S}_k$ directly is exponential in $K$, since the sum in \eqref{eq: augmented_sinkhorn_calculate_marginal} has an exponential number of terms.
Moreover, no \textit{general} polynomial-time algorithms for even approximating~\eqref{eq: augmented_sinkhorn_calculate_marginal} exist under standard computational complexity assumptions~\citep[Lemma 3.7]{AltBoi23}.
Together, these facts suggest that~\eqref{eq:eot_problem} will only be computationally feasible under special assumptions on $R$.
%%, for $\mu_k$ which are not necessarily absolutely continuous, we adopt the 
%The benefit of the static formulation in \cref{lem:dyn_to_stat} is that if the measures $\mu_k$ are supported on a finite set $\cX$, the joint measure $P_{[K]}$ can be represented by a finite---albeit exponentially large---order $(K+1)$ tensor, of total size $|\cX|^{K+1}$.

A crucial observation~\cite{AltBoi23,ChiZhaHei22}, which has driven the near-universal choice of Brownian motion as a prior, is that when $R$ is a \textit{Markov} process,~\eqref{eq: augmented_sinkhorn_calculate_marginal} can be computed in $\mathrm{poly}(K, |\cX|)$ time.
The tractability of marginalization when $R$ is a Markov process follows from the decomposition
\begin{equation*}
	\exp(-C(\bx) ) = R_{[K]}(\bx) = R_0(x_{0}) \prod_{k=1}^KR_{k \mid k-1}(x_{k} | x_{{k-1}})\,,
\end{equation*}
which shows that the exponential-size sum in~\eqref{eq: augmented_sinkhorn_calculate_marginal} factors into $K$ sums, each of which can be computed efficiently.
The assumption that $R$ is Markov extends even to works that consider priors other than Brownian motion~\cite{BunHsiCut23,VarThoLam21}.

This raises what appears to be an inherent tension: efficient algorithms for~\eqref{eq:eot_problem} rely on the assumption that the process $R$ is Markov; however, limiting to the case of Markov processes necessarily precludes consideration of priors $R$ with smooth sample paths (see Lemma \ref{lemma: Gauss-Markov Non-Diff}). %\footnote{For example, the only stationary Markov Gaussian process on $\bR$ is the Ornstein--Uhlenbeck process, whose sample paths are nowhere differentiable with probability $1$~\cite{RasWil06}.}
This observation suggests the pessimistic conclusion that \textit{no} practical algorithm exists for solving Schrödinger bridges with smooth priors.

However, the key contribution of this work is to show that this conclusion is \textit{false}.
The next section identifies a class of smooth priors for which~\eqref{eq:eot_problem} can be solved efficiently.
%
%The existence of an efficient algorithm for~\eqref{eq:eot_problem} when $R$ is a Markov process follows from the decomposition $$\log R_{[K]}(\bomega) = \log R_0(\omega_{0}) + \sum_{k=1}^K \log R_{k \mid k-1}(\omega_{k} | \omega_{{k-1}}),$$ which shows that the objective function in~\eqref{eq:eot_problem} is separable.
%This fact guarantees that the corresponding static problem decouples into $K$ separate optimization problems, each of size $O(|\cX|^2)$, which can then be solved in polynomial time~\cite{jason}.
%Below, we develop an approach with smooth priors that gives rise to a similar decomposition.
%\begin{align*}
%	C(\bomega) & = \log R_{[K]}(\bomega) \\
%	& = \log R_0(\omega_{t_0}) + \sum_{k=1}^K \log R_{k \mid k-1}(\omega_{t_k} | \omega_{t_{k-1}}) \\
%	& =: C_0(\omega_{t_0}) + \sum_{k=1}^K C_{k \mid k-1}(\omega_{t_k} | \omega_{t_{k-1}})
%\end{align*}
\subsection{Autoregressive Gaussian processes}
To develop our proposal for efficient smooth Schrödinger bridges, we focus on the class of \textit{continuous-time  Gaussian autoregressive processes}, a classic model in statistics and signal processing~\cite{Phi59}.
They are also a widespread choice in applications: as we show below (\cref{thm:gp}), the famous \textit{Matérn kernel} gives rise to such processes.
While it is known that such processes offer crucial efficiency benefits in Gaussian process regression~\cite{GilSaaCun15}, their algorithmic implications for the SB problem have not been explored prior to this work.
\begin{definition}[{\citealp[Appendix B]{RasWil06}}]
	Let $m$ be a positive integer.
	A Gaussian process $t \mapsto \omega(t)$ defined on $C^{m-1}(\bR; \bR^d)$ is a \textit{Gaussian autoregressive process} (GAP) of order $m$ if it is a stationary solution to the stochastic differential equation
	\begin{equation*}
		\frac{d^{m}}{d t^{m}} \omega(t) + a_{m-1} \frac{d^{m-1}}{d t^{m-1}} \omega(t) + \dots + a_0 \omega(t) =  \sigma \xi(t)\,,
	\end{equation*}
	for some constants $a_{0}, \dots, a_{m-1} \in \bR$ and $\sigma \in \bR^{d \times d}$, where $\xi(t)$ denotes a white-noise process on $\bR^d$ with independent coordinates.
\end{definition}

The key fact about GAPs, which we leverage to develop efficient algorithms, is that, even though a GAP $\omega$ is typically not Markov, the process $\eta := (\omega, d \omega/dt, \dots, d^{m-1} \omega/ dt^{m-1})$ taking values in phase space $\bR^{d \times m}$ \textit{is} a Markov process. We call $\eta$ the ``lifted'' Gaussian process corresponding to $\omega$.
The main observation driving our practical algorithm for smooth Schrödinger bridges is that when $R$ is a GAP, problem~\eqref{eq:eot_problem} admits an efficient algorithm obtained by \textit{lifting} the optimization problem to phase space.

GAPs form a rich class of smooth Gaussian processes.
Moreover, they admit a simple characterization in terms of their covariance functions.
Recall that a Gaussian process $\omega$ taking values in $C(\bR; \bR^d)$ is characterized by two functions $m: \bR \to \bR^d$ and $\kappa: \bR^2 \to \bR^{d \times d}$, which satisfy
\begin{equation*}
	m(t) = \bE \omega(t), \quad \quad \kappa(s, t)_{ij} = \operatorname{cov}(\omega(s)_i, \omega(t)_j)\,.
\end{equation*}
The process is \textit{stationary} if $\kappa(s, t) = k(t - s)$ for some $k: \bR \to  \bR^{d \times d}$.
For notational convenience, we focus on the zero-mean case, where $m \equiv 0$, though our results apply to the general case as well.
Zero-mean, stationary Gaussian processes are characterized entirely by the covariance function $k$.
 
We summarize the important properties of GAPs in the following theorem.

\begin{theorem}[{\citealp[Section 2.2]{Saa12}}]\label{thm:gp}
	Let $\omega$ be a zero-mean continuous, stationary Gaussian process on $\bR^d$ with covariance function $k$.
	Then $\omega$ is a GAP of order $m$ if and only if its spectral density $S_\omega(\tau) := \frac{1}{2 \pi }\int_{-\infty}^\infty k(t) e^{- i t \tau} d t \in \mathbb{C}^{d \times d}$ is of the form
	\begin{equation*}
		S_\omega(\tau) = \sigma \sigma^\tau/f(\tau^2)\,, \quad \quad \forall \tau \in \bR
	\end{equation*}
	where $f$ is a polynomial of degree $m$.
	
	Moreover, if $\omega$ is a GAP of order $m$, then $\eta := (\omega, d \omega/dt, \dots, d^{m-1} \omega/ dt^{m-1})$ is a zero-mean, stationary Gauss--Markov process.
\end{theorem}

With \cref{thm:gp} in hand, we easily obtain many examples of GAPs.
Crucially, this includes Gaussian processes corresponding to the Matérn kernel, the most popular smooth Gaussian process in applications, defined by the covariance function
\begin{equation}\label{eq:materncov}
	k(t) \propto \sigma^2(\sqrt{2 \nu} t/\ell)^\nu K_\nu(\sqrt{2 \nu} t/\ell)\,,
\end{equation}
where $K_\nu$ is the modified Bessel function of the second kind and $\nu$ and $\ell$ are positive parameters.
\begin{proposition}[{\citealp[Section 4.1]{HarSAr10}}]
	Suppose $\omega$ is a Gaussian process on $C(\bR; \bR)$ whose covariance function is a Matérn kernel for smoothness parameter $\nu = m - 1/2$, for $m \in \mathbb N$.
	Then $\omega$ is a GAP of order $m$.
\end{proposition}
By \cref{thm:gp}, the same holds true in the multidimensional case if each coordinate is taken to be independent of Matérn covariance.

Though the above characterization is formulated for stationary processes, our algorithm also applies to the nonstationary case, for instance, to the case of integrated Brownian motion: $\frac{d^{m}}{dt^{m}} \omega(t) = \sigma \xi(t)$.
Taking $m = 1$ recovers the standard Schr\"odinger bridge, and $m = 2$ gives rise to the so-called ``momentum Schr\"odinger bridge,'' previously studied in~\citep*{CheConGeo19,CheLiuTao23}.
The integrated Brownian motion prior possesses close connections to spline regression; see~\citep[Section 2.2.3]{Saa12} for more details. 

\section{Lifting Schrödinger Bridges}\label{sec:lifted}
The remainder of this paper is devoted to giving an efficient algorithm for smooth SBs whose reference process is a GAP.
In this section, we leverage the structure of GAPs to \textit{lift}~\eqref{eq:eot_problem} to a higher-dimensional problem, with better structure.
In Section~\ref{Sec: BP-continuous}, we show that this reformulated problem can be solved by a belief propagation algorithm in a number of iterations that scales \textit{linearly} with $K$.
Finally, in Section~\ref{sec:approx_bp}, we develop a practical approximation of the belief propagation algorithm, with overall runtime quadratic in $K$.

In what follows, for notational convenience, we focus on the case $d = 1$.
(We discuss the runtime considerations assciated with larger $d$ in Section~\ref{sec:practical}.)

Let $R$ be the law of a mean zero GAP $\omega$ of order $m$ for an integer $m > 0$.
\Cref{thm:gp} guarantees that $\eta := (\omega, d\omega/dt, \ldots, d^{m-1}\omega/dt^{m-1})$ is a stationary Gauss--Markov process on $\bR^{m}$, whose law we denote by $\tilde R$.
We write $\tilde R_{[K]}$ for the joint law of the finite-dimensional vector $\bdeta := (\eta_{0}, \dots, \eta_{K})$, which is Gaussian with mean $0$ and covariance matrix $\tilde \Sigma \in \bR^{m(K+1) \times m(K+1)}$.

We first show that the smooth Schrödinger bridge problem corresponding to $R$ can be rewritten in terms of $\tilde R$.
Suppose for concreteness that $\mu_k$ is supported on a finite set $\cX_k \subseteq \bR$, and write $\cX_{[K]} = \prod_{k=0}^K \cX_k$.
We write $\cY_{[K]} := \bR^{(m-1)(K+1)}$.
Given a probability measure $\tilde P$ on phase space $\cZ_{[K]} := \cX_{[K]} \times \cY_{[K]}$ whose marginal distribution on $\cY_{[K]}$ is absolutely continuous, we write $p(\bx, \by)$ for its density with respect to the product of the counting measure on $\cX_{[K]}$ and the Lebesgue measure on $\cY_{[K]}$.
We will use the variable $\bz = (\bx, \by)$ to denote an element of $\cZ_{[K]}$.

We obtain the following:
\begin{lemma}\label{lem:eot_to_lifted}
		There is a one-to-one correspondence between solutions to~\eqref{eq:eot_problem} and solutions to
	\begin{equation}
		\min_{p} \frac 12 \int_{\cY_{[K]}} \sum_{\bx \in \cX_{[K]}} \bz^\top \tilde \Sigma^{-1} \bz \, p(\bz)\, d \by - \cH(p),~~ %+ \int_{\cY_{[K]}} \sum_{\bx \in \cX_{[K]}} p(\bz) \log p(\bz) \, d\bz\,, \\
		p_{x_k} = \mu_k,~~\forall k \in [K], \label{eq:lifted_eot}
	\end{equation}
	where $\cH(p) := - \int_{\cY_{[K]}} \sum_{\bx \in \cX_{[K]}} p(\bz) \log p(\bz) \, d\by$  and the minimization is taken over all densities on  $\cZ_{[K]}$ under which the marginal law of $x_k$ is equal to $\mu_k$. 
\end{lemma}
We refer to~\eqref{eq:lifted_eot} as the \emph{lifted} Schr\"odinger Bridge problem, since it is obtained by lifting the optimization problem from densities on $\cX_{[K]}$ to densities on $\cZ_{[K]}$.

At first sight, the lifted problem~\eqref{eq:lifted_eot} is no improvement over~\eqref{eq:eot_problem}---indeed, the situation seems to have become worse due to the introduction of the continuous variables $\by$.
However, we now show that unlike~\eqref{eq:eot_problem},  problem~\eqref{eq:lifted_eot} is directly amenable to efficient algorithms.

The first step is to leverage the Gauss--Markov property of $\tilde{R}_{[K]}$ to simplify~\eqref{eq:lifted_eot}.
Recall the fundamental fact that, under $\tilde R$, the law of $\bdeta$ has the Markov property.
Given $\bz = (\bx, \by) \in \cZ_{[K]}$ and $k \in [K]$, we write $\bz_k = (x_k, \by_k)$ for the $k$th coordinate of $\bz$, which takes values in $\cZ_{k}$.
The Markov property then implies that $\bz_{k+1}$ is independent of $\bz_0, \dots, \bz_{k-1}$, conditioned on $\bz_k$.
At the level of densities, this implies the decomposition
\begin{equation}
	\begin{aligned}\label{eq:r_fac}
			 r(\bz) & =
		r(\bz_0) \prod_{k=1}^{K} r(\mathbf{z}_{k} | \mathbf{z}_{k-1}) \\
		& \propto r(\bz_0) \prod_{k=1}^K \exp\left(- \frac 12 Q_k(\bz_{k-1}, \bz_k)\right)\,,
		%	 
		%	 
		%	 \exp\left(-\frac{1}{2} \mathbf{z}_{0}^K \tilde \Sigma_{0, 0}^{-1} \mathbf{z}_0\right)  \cdot \\
		%	\prod_{k=0}^{K-1} \exp\left(-\frac{1}{2} (\mathbf{z}_{k+1} - A_k \mathbf{z}_k)^K \Lambda_k^{-1} (\mathbf{z}_{k+1} - A_k \mathbf{z}_k) \right),
	\end{aligned}
\end{equation}
where $r(\bz_0) \propto \exp(- \tfrac 12 \bz_0^\top \tilde \Sigma_{0, 0}^{-1} \bz_0)$ and each $Q_k$ is a quadratic function:
\begin{align*}
%Q_1(\mathbf{z}_{0}, \bz_1) &:= \bz_0^\top \tilde \Sigma_{0, 0}^{-1} \bz_0 + (\mathbf{z}_{1}{-}A_0 \mathbf{z}_0)^T \Lambda_0^{-1} (\mathbf{z}_{1}{-}A_0 \mathbf{z}_0) \nonumber\\
Q_k(\mathbf{z}_{k-1}, \bz_{k}) &:= (\mathbf{z}_{k}{-}A_k \mathbf{z}_{k-1})^T \Lambda_k^{-1} (\mathbf{z}_{k}{-}A_k \mathbf{z}_{k-1})\,, 
\end{align*}
for matrices
$A_k := \tilde{\Sigma}_{k,k-1} (\tilde{\Sigma}_{k-1, k-1})^{-1} \in \bR^{m \times m}$ and $\Lambda_k := \tilde{\Sigma}_{k, k} - \tilde{\Sigma}_{k, k-1} (\tilde{\Sigma}_{k-1, k-1})^{-1} \tilde{\Sigma}_{k-1, k} \in \bR^{m \times m}$.
These representations follow directly from standard formulas for Gaussian conditioning, and admit explicit expressions in terms of the kernel $k$ of the GAP~\citep[Section 2.3.1]{Saa12}.


% Therefore, problem \eqref{obj: aug_schrodinger} can be reformulated as the following entropy-regularized optimal transport problem:
% \begin{align}
%     &\min_{p}  \int_{\mathbb{R}^{(m-1)(K+1)}} \sum_{\mathbf{x} \in \mathcal{X}_{[K]}} p(\mathbf{z}) c(\mathbf{z}) d\mathbf{z} - \mathcal{H}(p) \label{obj: augmented_optimal_transport} \\
%     &\hspace{15mm} \text{s.t.} \ p_{\omega_{t_{k}}} = \mu_k, \forall k \in \{ 0, ..., K \} \label{constrain: augmented_optimal_transport}
% \end{align}
% where the minimization is over all probability distributions on $\mathcal{X}_{[K]} \times \mathbb{R}^{(m-1)(K+1)}$, which are continuous on $\mathbb{R}^{(m-1)(K+1)}$. Moreover, the entropy $\mathcal{H}(p)$ is given by
% \begin{align}
%     \mathcal{H}(p) &:= - \int_{\mathbb{R}^{(m-1)(K+1)}} \sum_{\mathbf{x} \in \mathcal{X}_{[K]}} p(\mathbf{z}) \log p(\mathbf{z}) d\mathbf{z},
% \end{align}
% and the cost function $c(\mathbf{z})$ is given by
%Therefore, we can rewrite the first term in \eqref{eq:lifted_eot} as 
%\begin{align}
%    \frac 12 \bz^\top \tilde \Sigma^{-1} \bz = \frac{1}{2} \sum_{k = 0}^{K-1} Q_k(\mathbf{z}_k, \mathbf{z}_{k+1}), 
%\end{align}
%where
%\begin{align}
%    Q_0(\mathbf{z}_{0:1}) &:= \bz_0^\top \tilde \Sigma_{0, 0}^{-1} \bz_0 + (\mathbf{z}_{1}{-}A_0 \mathbf{z}_0)^K \Lambda_0^{-1} (\mathbf{z}_{1}{-}A_0 \mathbf{z}_0) \nonumber\\
%    Q_k(\mathbf{z}_{k:k+1}) &:= (\mathbf{z}_{k{+}1}{-}A_k \mathbf{z}_k)^K \Lambda_k^{-1} (\mathbf{z}_{k{+}1}{-}A_k \mathbf{z}_k)\,, \,\, k \geq 1 \nonumber
%\end{align}

This decomposition represents the first term in~\eqref{eq:lifted_eot} as a ``tree-structured cost''~\cite{HaaRinChe21}, therefore rendering the marginalization in~\eqref{eq: augmented_sinkhorn_calculate_marginal} amenable to belief propagation methods.
We develop such a method in the next section.


% In the next section, we show that seeking a minimizer to \eqref{obj: augmented_optimal_transport}-\eqref{constrain: augmented_optimal_transport} is equivalent to seeking a minimizer of the free energy on a probabilistic graphical model with factor node potentials given by factors of $q$. This interpretation eventually leads us to a message-passing algorithm. 

\begin{figure}
    \centering
\begin{tikzpicture}[
	scale=0.6,
	every node/.style={scale=0.6},
	circlenode/.style={circle, draw, minimum size=0.8cm, inner sep=0pt},
	squarenode/.style={rectangle, draw, minimum size=0.8cm, inner sep=0pt}
	]
	
	% Define the main nodes
	\node[circlenode] (eta_k1) {$\eta_{k-1}$};
	\node[squarenode] (alpha_k1) [below=0.7cm of eta_k1] {$\alpha_{k-1}$};
	\node[circlenode] (omega_k1) [below=0.7cm of alpha_k1] {$\omega_{k-1}$};
	
	\node[squarenode] (alpha_k1k) [right=1.5cm of eta_k1] {$\alpha_{k-1,k}$};
	
	\node[circlenode] (eta_k) [right=1.5cm of alpha_k1k] {$\eta_k$};
	\node[squarenode] (alpha_k) [below=0.7cm of eta_k] {$\alpha_k$};
	\node[circlenode] (omega_k) [below=0.7cm of alpha_k] {$\omega_k$};
	
	% Add the arrows between vertical nodes (eta_k1 <-> alpha_k1)
%	\draw[->, shorten >=2pt, shorten <=2pt] (eta_k1) -- node[left] {$m_{\alpha_{k-1}\to\eta_{k-1}}$} (alpha_k1);
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k1) -- node[left] {$\upmesskminus$} (eta_k1);
	
	% Add the arrows between vertical nodes (alpha_k1 <-> omega_k1)
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k1) -- node[left] {$\downmesskminus$} (omega_k1);
%	\draw[->, shorten >=2pt, shorten <=2pt] (omega_k1) -- node[right] {$n_{\omega_{k-1}\to\alpha_{k-1}}$} (alpha_k1);
	
	% Add the arrows between eta_k1 and alpha_k1k
%	\draw[->, shorten >=2pt, shorten <=2pt] (eta_k1) -- node[above] {$n_{\eta_{k-1}\to\alpha_{k-1,k}}$} (alpha_k1k);
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k1k) -- node[above] {$\leftmesskminus$} (eta_k1);
	
	% Add the arrows between alpha_k1k and eta_k
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k1k) -- node[above] {$\rightmessk$} (eta_k);
%	\draw[->, shorten >=2pt, shorten <=2pt] (eta_k) -- node[below] {$n_{\eta_k\to\alpha_{k-1,k}}$} (alpha_k1k);
	
	% Add the arrows between vertical nodes (eta_k <-> alpha_k)
%	\draw[->, shorten >=2pt, shorten <=2pt] (eta_k) -- node[left] {$m_{\alpha_k\to\eta_k}$} (alpha_k);
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k) -- node[right] {$\upmessk$} (eta_k);
	
	% Add the arrows between vertical nodes (alpha_k <-> omega_k)
	\draw[->, shorten >=2pt, shorten <=2pt] (alpha_k) -- node[right] {$\downmessk$} (omega_k);
%	\draw[->, shorten >=2pt, shorten <=2pt] (omega_k) -- node[right] {$n_{\omega_k\to\alpha_k}$} (alpha_k);
	
	% Add the dots on both sides
	\node[left=0.3cm of eta_k1] {$\cdots$};
	\node[right=0.3cm of eta_k] {$\cdots$};
	
	% Add horizontal arrows to dots
	\draw[<-,  shorten <=2pt] ($(eta_k1.west)+(0,0)$) -- ++(-0.4,0);
	\draw[<-, shorten <=2pt] ($(eta_k.east)+(0,0)$) -- ++(0.4,0);
	
\end{tikzpicture}
     \label{fig: HMM}
     \caption{A portion of the graphical model corresponding to the joint law of $\bomega$ and $\bdeta$.}
\end{figure}

\section{Belief Propagation} \label{Sec: BP-continuous}
The goal of this section is to show that a \textit{belief propagation} algorithm can be used to efficiently solve the lifted problem~\eqref{eq:lifted_eot}.
Belief propagation~\cite{KscFreLoe01,Pea82} is a canonical approach for performing inference in high-dimensional models whose densities possess simple factorizations, such as the one given in~\eqref{eq:r_fac}.
The use of belief propagation algorithms for Sinkhorn-type problems is not new~\cite{HaaRinChe21,SinZhaChe22,TehWel01}; however, we stress that their application to Schr\"odinger bridges with smooth priors is novel.

To develop our algorithm, we first reformulate~\eqref{eq: augmented_sinkhorn_calculate_marginal} in the language of graphical models.
\citep[See][for background.]{KolFri09,WaiJor07}
The probabilistic structure of  $\bomega$ and the lifted process $\bdeta$ under $\tilde R$ means that we can represent their joint distribution by a simple hidden Markov model (see Figure \ref{fig: HMM}), with observed variables $\{ \omega_{k} \}_{k = 0}^{K}$ and hidden variables $\{ \eta_{k} \}_{k=0}^{K}$.
These correspond to \textit{variable nodes} in \cref{fig: HMM}, denoted by circles.

The dependencies among these variables nodes are represented by \textit{factor nodes} (squares in Figure~\ref{fig: HMM}): the factor nodes $\alpha_{k-1, k}$ connecting $\eta_{k-1}$ and $\eta_{{k}}$ enforce the joint law of the pair $(\eta_{k}, \eta_{{k+1}})$, and the factor nodes $\alpha_{k}$ connecting $\eta_{k}$ and $\omega_{k}$ enforce the deterministic requirement that the first coordinate of $\eta_{k}$ equals $\omega_{k}$.
We associate to $\alpha_{k-1, k}$ the \textit{factor node potential} $\Phi_{k}: \cZ_{k-1} \times \cZ_k$ given by
\begin{align*}
	\Phi_1(\mathbf{z}_0, \mathbf{z}_1) & :=  \exp \left( -\frac{\bz_0^\top \tilde \Sigma_{0, 0}^{-1} \bz_0 + Q_{1}(\mathbf{z}_{0}, \mathbf{z}_{1})}{2} \right) \\
    \Phi_{{k}}(\mathbf{z}_{k-1}, \mathbf{z}_{k})  & := \exp \left( -\frac{Q_{k}(\mathbf{z}_{k-1}, \mathbf{z}_{k})}{2} \right) \quad k > 1,
%    \Psi_{k}(o_k, x_k, \mathbf{y}_k) & := \bone_{o_k}(x_k).
\end{align*} 
so that
%In terms of these potentials, the joint density of the pair $(\bomega,\bdeta)$ on $\cX_{[K]} \times \cZ_{[K]}$ under $\tilde{R}$ is
\begin{equation*}
	r(\bz) \propto \prod_{k=1}^{K} \Phi_{k}(\bz_{k-1}, \bz_{{k}}) \,.
\end{equation*}

%Writing $\bo$ and $\bz = (\bx, \by)$ for dummy variables on $\cX_{[K]}$ and $\cZ_{[K]}$, respectively, we obtain that the objective in~\eqref{eq:lifted_eot} is equivalent to the free energy $\mathcal{F}_{\mathrm{free}}(p)$ of a probability density $p$ on $\cX_{[K]} \times \cZ_{[K]}$, defined by
%\begin{multline}
% \mathcal{F}_{\mathrm{free}}(p) =\\ - \int_{\cY_{[K]}} \sum_{\mathbf{o}, \bx \in \mathcal{X}_{[K]}} p(\mathbf{o}, \mathbf{z}) \sum_{k=0}^{K-1} \log \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) d\mathbf{y}   \\
% -\int_{\cY_{[K]}} \sum_{\mathbf{o}, \bx \in \mathcal{X}_{[K]}} p(\mathbf{o}, \mathbf{z}) \sum_{k=0}^{K} \log \Psi_{k}(o_k, \mathbf{z}_k) d\mathbf{y} \label{eq: free_energy} \\
% +\int_{\cY_{[K]}} \sum_{\mathbf{o}, \bx \in \mathcal{X}_{[K]}} p(\mathbf{o}, \mathbf{z}) \log p(\mathbf{o}, \mathbf{z}) d\mathbf{y}. 
%\end{multline}

%\jnw{I am leaving the next several paragraphs in blue for Yuliang to edit.}

%{\color{blue}
%Since the factor graph is a tree, it is known that \jnw{Insert citation/justification} the minimizer $p^*$ of~\eqref{eq:eot_problem} can be written 
%\begin{align}
%    p^*(\mathbf{o}, \mathbf{z}) \ = \ \frac{\prod_{k=0}^{K-1} p_{\alpha_{k, k+1}}^*(\mathbf{z}_k, \mathbf{z}_{k+1}) \prod_{k=0}^{K} p_{\alpha_k}^*(o_k, \mathbf{z}_k) }{p_{\eta_0}^*(\mathbf{z}_0) \prod_{k=1}^{K-1} p_{\eta_k}^*(\mathbf{z}_k)^2 \ p_{\eta_K}^*(\mathbf{z}_K)}. \label{eq: tree_decomposition_of_density}\,,
%\end{align}
%for suitable functions $p_{\alpha_{k, k+1}}$, $p_{\alpha_k}^*$, and $p_{\eta_k}$.
%Therefore, we can restrict the optimization domain to the set of probability densities that possess relation \eqref{eq: tree_decomposition_of_density} between the joint and the marginals. After replacing $\log p(\mathbf{o}, \mathbf{z})$ with \eqref{eq: tree_decomposition_of_density} in the last line of \eqref{eq: free_energy}, we obtain the Bethe free energy $\mathcal{F}_{\mathrm{Bethe}}(\{ p_{\alpha_{k, k+1}} \} \cup \{p_{\alpha_k} \} \cup \{ p_{\eta_k}\})$ as a function taking factor and variable node marginals as input. Moreover, the minimization task is subject to the following marginalization constraints:
%\begin{align}
%    &\int \sum_{x_k} p_{\alpha_{k, k+1}}(\mathbf{z}_k,\mathbf{z}_{k+1}) d\mathbf{y}_k = p_{\eta_{k+1}}(\mathbf{z}_{k+1}), \label{constraints: bethe_free_energy_1}\\
%    &\int \sum_{x_{k+1}} p_{\alpha_{k, k+1}}(\mathbf{z}_k, \mathbf{z}_{k+1}) d\mathbf{y}_{k+1} = p_{\eta_{k}}(\mathbf{z}_{k}), \label{constraints: bethe_free_energy_2}\\
%    &\sum_{o_k} p_{\alpha_k}(o_k, \mathbf{z}_k) = p_{\eta_k}(\mathbf{z}_k), \label{constraints: bethe_free_energy_3}\\
%    &\int \sum_{x_k} p_{\alpha_k}(o_k, \mathbf{z}_k) d\mathbf{y}_k = \mu_k(o_k), \label{constraints: bethe_free_energy_4}
%\end{align}
%where \eqref{constraints: bethe_free_energy_1}-\eqref{constraints: bethe_free_energy_2} holds for $k = 0, ..., K-1$ while \eqref{constraints: bethe_free_energy_3}-\eqref{constraints: bethe_free_energy_4} holds for $k = 0, ..., K$. }


To find the optimal solution $p^*$ to~\eqref{eq:lifted_eot}, we use a belief propagation algorithm (\cref{alg: BP-continuous}).
The algorithm iteratively updates ``messages'' traveling between factor and variable nodes, which are depicted in Figure~\ref{fig: HMM}.
The ``vertical'' messages $\upmessk$, $\downmessk$ are real-valued functions on $\cX_k$ which encode information about the $\bomega$ marginals of $p^*$, while the ``horizontal'' messages $\leftmessk$, $\rightmessk$ are real-valued functions on $\cZ_k$ which encode information about the joint distribution of $\eta_k$ and its neighbors $\eta_{k-1}$ and $\eta_{k+1}$
These messages are iteratively updated back and forth across the graph via the application of the following operators:



\begin{equation}\label{eq:operators}
\begin{aligned}
%		\mathcal{L}(n)(\mathbf{z}_k) & := \mathcal{L}(n)(x_k, \mathbf{y}_k) = n(x_k) \\
\updownkop(\rightmessk, \leftmessk)(x_k) :&= \int_{\cY_k} \rightmessk(x_k, \by_k) \leftmessk(x_k, \by_k) d \by_k\\
\leftkop(\leftmessk,\upmessk)(\bz_{k-1}) :&= \sum_{x_{k} \in \cX_{k}} \int_{\cY_{k}} \Phi_{k}(\bz_{k-1}, \bz_{k}) \leftmessk(\bz_k) \upmessk(x_k) d \by_{k}\\
\rightkminusop(\rightmesskminus,\upmesskminus)(\bz_{k}) :&= \sum_{x_{k-1} \in \cX_{k-1}} \int_{\cY_{k-1}} \Phi_{k}(\bz_{k-1}, \bz_{k}) \rightmessk(\bz_{k-1}) \upmessk(x_{k-1}) d \by_{k-1} 
%		\mathcal{I}_{\Phi_{k}}^{(1)}(n)(\mathbf{z}_{k+1})& := \sum_{x_{k}} \int \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) n(\mathbf{z}_k) d\mathbf{y}_k, \\
%		\mathcal{I}_{\Phi_{k}}^{(2)}(n)(\mathbf{z}_{k}) &:= \sum_{x_{k+1}} \int \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) n(\mathbf{z}_{k+1}) d\mathbf{y}_{k+1}, \\
%		\mathcal{I}_{\Psi}(n)(x_k) &:= \int n(x_k, \mathbf{y}_k) d\mathbf{y}_k.
\end{aligned}
\end{equation}



Since these operators involve manipulating functions on the space $\cZ_k$, they are not directly implementable.
In this section, we regard these operators as single basic operators for the purpose of complexity analysis.
We develop efficient techniques to bypass their direct evaluation in the next section.

%
%We first analyze the fixed points of \cref{alg: BP-continuous} and show that they coincide with optimal solutions to~\eqref{eq:lifted_eot}.
%
%\begin{theorem} \label{thm: fixed_point_theorem}
%    The optimal probability distributions $p_{\alpha_{k, k+1}}$, $p_{\alpha_k}$, and $p_{\eta_k}$ to minimize $\mathcal{F}_{\mathrm{Bethe}}(\{ p_{\alpha_{k, k+1}} \} \cup \{p_{\alpha_k} \} \cup \{ p_{\eta_k}\})$, subject to constraints \eqref{constraints: bethe_free_energy_1}-\eqref{constraints: bethe_free_energy_4} must satisfy that $p_{\alpha_{k, k+1}}(\mathbf{z}_k, \mathbf{z}_{k+1})$ is proportional to
%\begin{equation}
%    \begin{aligned}
%    \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) n^*_{\eta_k \to \alpha_{k,k+1}}(\mathbf{z}_k) n^*_{\eta_{k+1} \to \alpha_{k,k+1}}(\mathbf{z}_{k+1}), \label{eq: Belif_alpha_tt+1} 
%     \end{aligned}
%\end{equation}
%$p_{\eta_k}(\mathbf{z}_k)$ is proportional to 
%\begin{equation}
%    \begin{aligned}
%	m^*_{\alpha_{k,k+1} \to \eta_k}(\mathbf{z}_k) m^*_{\alpha_{k-1,k} \to \eta_k}(\mathbf{z}_k)  m^*_{\alpha_{k} \to \eta_k}(\mathbf{z}_k), \label{eq: Belif_Z_t}
%    \end{aligned}
%\end{equation}
%and $p_{\alpha_k}(o_k, \mathbf{z}_k)$ equals to $p_{\eta_k}(\mathbf{z}_k)$ whenever $o_k = x_k$ and equals to 0 otherwise, where the messages  $m^*$ and $n^*$ constitutes a set of fixed points of Algorithm \ref{alg: BP-continuous}.
%\end{theorem}

The main result of this section is that Algorithm~\ref{alg: BP-continuous} implicitly implements the Sinkhorn algorithm (Algorithm~\ref{alg: Multi_Sinkhorn}) for the multi-marginal entropic optimal transport problem~\eqref{eq:eot_problem}, with cost given by
\begin{equation}
	\exp(-C(\bx)) = \idotsint \prod_{k=1}^{K} {\Phi}_{k}(\bz_{k-1}, \bz_{k}) d\by_0 \cdots d \by_K\,. \label{eq:bp_to_sink_connection}
\end{equation}
This connection allows us to develop a rigorous convergence guarantee for Algorithm~\ref{alg: BP-continuous}.
Indeed, \eqref{eq:bp_to_sink_connection} implies that $\exp(-C(\bx))$ is, up to a normalizing constant, the joint density of $R_{[K]}$, so that Algorithm~\ref{alg: Multi_Sinkhorn}, and hence Algorithm~\ref{alg: BP-continuous}, solves the smooth Schrödinger Bridge problem.



\begin{algorithm}[h]
\begin{algorithmic}[1]
\STATE \textbf{Input:} Factor node potentials $\{ \Phi_k \}_{k=0}^{K-1}$, distributions $\{\mu_k\}_{k=0}^{K}$ on $\{ \mathcal{X}_{k} \}_{k = 0}^{K}$.


%\vspace{2mm}
%\COMMENT{\textit{Initialization}}
%\STATE Set $m^{(\ell)}_{\alpha_{\alpha_{-1, 0}} \rightarrow \eta_0} = m^{(\ell)}_{\alpha_{\alpha_{K, K+1}} \rightarrow \eta_K} \equiv 1$ for all $\ell$.
\STATE Initialize $\ell = 0$, $\leftmessend \equiv 1$, $\rightmessend \equiv 1$, and $\upmessk^{(0)} : \cX_k \to \bR^+$, $k \in [K]$ arbitrary
\WHILE{not converged}
\STATE $\ell \gets \ell + 1$

% \COMMENT{\textit{/* left pass */}}
\FOR[\textit{/* left pass */}]{$k = K, ..., 1$}
%\COMMENT{\textit{/* update vertical messages */}}
%\STATE $\downmessk^{(\ell)} \gets \updownkop(\rightmessk, \leftmessk)$ \label{alg_line: BP_cont_integrate}
%\STATE $\upmessk^{(\ell)} \leftarrow \mu_k \oslash \downmessk^{(\ell)} $
\STATE $\leftmesskminus \gets \leftkop(\leftmessk, \upmessk^{(\ell-1)})$
%\COMMENT{bad below}
%\STATE $m^{(\ell-1)}_{\alpha_T \rightarrow \eta_T} \leftarrow \mathcal{L}(n^{(\ell-1)}_{\omega_{T} \rightarrow \alpha_{T}})$ 
%
%    \STATE $n^{(\ell)}_{\eta_k \rightarrow \alpha_{k-1, k}} \leftarrow m^{(\ell)}_{\alpha_{k, k+1} \rightarrow \eta_k} \odot m^{(\ell-1)}_{\alpha_{k} \rightarrow \eta_{k}}$ \label{alg_line: BP_cont_multiply-1}
%    \STATE $m^{(\ell)}_{\alpha_{k-1, k} \rightarrow \eta_{k-1}} \leftarrow \mathcal{I}^{(2)}_{\Phi_{k-1}} (n^{(\ell)}_{\eta_{k} \rightarrow \alpha_{k-1, k}})$ \label{alg_line: BP_cont_integrate-1}
\ENDFOR
\vspace{2mm}
\STATE $\downmesszero^{(\ell)} \gets \updownzeroop(\rightmessend, \leftmesszero)$
\STATE $\upmesszero^{(\ell)} \leftarrow \mu_0 \oslash \downmesszero^{(\ell)} $
%\STATE $n^{(\ell)}_{\eta_0 \rightarrow \alpha_0} \leftarrow m^{(\ell)}_{\alpha_{0, 1} \rightarrow \eta_0}$
%\STATE $m^{(\ell)}_{\alpha_0 \rightarrow \omega_0} \leftarrow \mathcal{I}_{\Psi}(n^{(\ell)}_{\eta_0 \rightarrow \alpha_0})$
%\STATE $n^{(\ell)}_{\omega_0 \rightarrow \alpha_0} \leftarrow \mu_0 \oslash m^{(\ell)}_{\alpha_0 \rightarrow \omega_0}$

\vspace{2mm}
\FOR[\textit{/* right pass */}]{$k = 1, ..., K$}
\STATE $\rightmessk \gets \rightkminusop(\rightmesskminus, \upmesskminus^{(\ell)})$
\STATE $\downmessk^{(\ell)} \gets \updownkop(\rightmessk, \leftmessk)$
\STATE $\upmessk^{(\ell)} \leftarrow \mu_k \oslash \downmessk^{(\ell)} $
\ENDFOR
\vspace{2mm}
\ENDWHILE
\STATE Return $(\upmessk^{(\ell)})_{k \in [K]}$
\end{algorithmic}
\caption{Belief Propagation with Continuous Massages} \label{alg: BP-continuous}
\end{algorithm}

%Given messages $\{n_{\omega_k \rightarrow \alpha_k}\}_{k \in [T]}$, we define the corresponding stochastic tensor by
%\begin{equation}
%\begin{aligned}
%& \hspace{10mm} P(x_0, ..., x_K) \\
%:= & \int \prod_{k = 0}^{K-1} \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) \prod_{k = 0}^{K} n_{\omega_k \rightarrow \alpha_k} (x_k) d\mathbf{y}.
%\end{aligned}
%\end{equation}
%The tensor $P$ is a multidimensional array of size $n^{K+1}$ and can be viewed as an element of $\cP_{\cX_{[K]}}$.
%\jnw{Wordsmith this}
{
%\begin{definition}[$\epsilon$-Approximate Solution]
%   Let $\mathcal{F}$ be the objective function given in \eqref{eq:eot_problem} and let $\mathcal{F}^*$ be the minimal value of $\mathcal{F}$. We say a stochastic tensor $P \in \mathcal{P}(\mathcal{X}_{[K]})$ is an $\epsilon$-approximate solution to \eqref{eq:eot_problem} if it satisfies that
%   \begin{align*}
%    \mathcal{F}(P) \le \mathcal{F}^* + \epsilon.
%    \end{align*}
%\end{definition}
\begin{theorem} \label{thm: poly_time_epsilon_approx}
    Algorithm \ref{alg: BP-continuous} is equivalent to Algorithm~\ref{alg: Multi_Sinkhorn} with cost given by~\eqref{eq:bp_to_sink_connection}, in the sense that,
    if the initialization of Algorithm \ref{alg: BP-continuous} and Algorithm \ref{alg: Multi_Sinkhorn} satisfy
\begin{align}
    \upmessk^{(0)} = v_k^{(0)} \quad \forall k \in [K]
\end{align}
then, for all $\ell \ge 0$ and all $k = 0, ..., K$, we have
\begin{align}
    \downmessk^{(\ell)} &= \mathbf{S}^{(\ell)}_k,
    \upmessk^{(\ell)} = v^{(\ell)}_k.
\end{align} 
In particular, we have the following two consequences:

(1) Algorithm \ref{alg: BP-continuous} achieves an $\epsilon$-approximate solution for \eqref{eq:eot_problem} in $\tilde O(K C_{\max} / \epsilon^{-1})$ iterations, where $C_{\max} = \max_{\bx \in \cX_{[T]}} C(\bx)$ and $\tilde O(\cdot)$ hides polylogarithmic factors in the problem parameters.

(2) The solution of \eqref{eq:lifted_eot} is given by 
\begin{equation}
    \begin{aligned}
        p(\bz) \propto \prod_{k = 1}^{K} \Phi_{k}(\mathbf{z}_{k-1}, \mathbf{z}_{k}) \prod_{k = 0}^{K} \upmessk^* (x_k) \label{eq: full_decomposition_p^*}
    \end{aligned}
\end{equation}
where $(\upmessk^*)_{k \in [K]}$ is the fixed point of Algorithm \eqref{alg: BP-continuous}.
%, which further implies that $p(\bz_k, \bz_{k+1})$ is proportional to
%\begin{equation}
%	{\color{red}
%    \begin{aligned}
%         \Phi_{k}(\mathbf{z}_k, \mathbf{z}_{k+1}) n^*_{\eta_k \to \alpha_{k,k+1}}(\mathbf{z}_k) n^*_{\eta_{k+1} \to \alpha_{k,k+1}}(\mathbf{z}_{k+1}). \label{eq: construct_B_using_message}
%    \end{aligned}}
%\end{equation}
\end{theorem}}

The representation in~\eqref{eq: full_decomposition_p^*} implies that the output of \cref{alg: BP-continuous} can be used to efficiently manipulate and sample from the solution to the smooth SB problem; see \cref{sec:sampling} for details.


\section{Approximate Belief Propagation}\label{sec:approx_bp}
The final ingredient of our algorithm is an approximation scheme to efficiently implement the operators in~\eqref{eq:operators}.
We use the technique proposed by~\cite{NooWai13}: we decompose the continuous messages in a suitable orthonormal basis.
The orthonormal decomposition method provides two key benefits: First, by truncating the series at a sufficiently high order, we can create an accurate representation of the messages using only a finite number of orthogonal coefficients. Second, the key update rules in Algorithm \ref{alg: BP-continuous} described in~\eqref{eq:operators} involve taking the $L^2$ inner product of two continuous messages.
Expressing the messages in an orthonormal basis simplifies these operations considerably.

Let $\{ \phi_k^i \}_{i=0}^{\infty}$ represent an orthonormal basis in the space $L^2(\mathbb{R}^{m-1})$.
The subscript $k$ indicates that one is free to choose different bases for different $k \in [K]$.

We express the horizontal messages $\leftmessk$ and $\rightmessk$ in terms of this basis as follows:
\begin{align}
    \leftmessk(\mathbf{z}_k) & = \sum_{i=1}^{\infty} \ell_{k}^{i}(x_k) \phi_k^{i}(\mathbf{y}_k), \label{approx: left}\\
    \rightmessk(\mathbf{z}_{k}) & = \sum_{i=1}^{\infty} r_{k}^{i} (x_{k}) \phi_{k}^{i}(\mathbf{y}_{k}), \label{approx: right}
\end{align}
where $r$ and $\ell$ denote the coefficients for rightward and leftward messages and the coefficients are given by 
\begin{align*}
    \ell^i_k(x_k) &:= \int \leftmessk(x_k, \mathbf{y}_k) \phi_k^i(\mathbf{y}_k) d\mathbf{y}_k \\
    r^i_{k}(x_{k}) &:= \int \rightmessk(x_{k}, \mathbf{y}_{k}) \phi_{k}^i(\mathbf{y}_{k}) d\mathbf{y}_{k},
\end{align*}
Utilizing the orthonormal expansions from \eqref{approx: left}-\eqref{approx: right}, we can re-write Algorithm \ref{alg: BP-continuous} so that it operates directly on the coefficients $\bl_k := (\ell_k^i)_{i=0}^\infty$ and $\br_k:= (r_k^i)_{i=0}^\infty$, which are functions from $\cX_k$ to $\ell_2$.

First, by $L^2(\cY_k)$ orthogonality, the update rule for $\downmessk$ can be written
\begin{align*}
	\updownkop(\leftmessk, \rightmessk)(x_k) %& = \int_{Y_k} \left(\sum_{i=1}^{\infty} \ell_{k}^{i}(x_k) \phi_k^{i}(\mathbf{y}_k)\right)\left(\sum_{i=1}^{\infty} r_{k}^{i}(x_k) \phi_k^{i}(\mathbf{y}_k)\right) d \by_{k} \\
	& = \langle \bl(x_k), \br(x_k) \rangle.
\end{align*}
Note that in this notation, we can write
\begin{equation*}
	\upmessk(x_k) = \mu_k(x_k)/\downmessk(x_k) = \mu_k(x_k) \langle \bl(x_k), \br(x_k) \rangle^{-1}
\end{equation*}

We now consider the update rule for the left and right messages.
The following lemma shows how to express these updates in terms of coefficients.
\begin{lemma}\label{lem:messages}
	Fix functions $\leftmessk = \sum_{i=1}^{\infty} \ell_{k}^{i} \otimes \phi_k^{i}$ and $\upmessk$.
	Then the coefficients of $\leftmesskminus = \leftkop(\leftmessk, \upmessk)$ in the basis $(\phi_{k-1}^i)_{i=1}^\infty$ are given by
	\begin{equation}
		\ell_{k-1}^i(x_{k-1}) = \sum_{x_k \in \cX_k} \upmessk(x_k) \sum_{j=1}^\infty \ell_k^j(x_k) 	\Gamma^{ij}_{k-1}(x_{k-1}, x_{k})\,,
	\end{equation}
	where $\Gamma^{ij}_{k-1}(x_{k-1}, x_{k})$ denotes
	\begin{equation}
		\iint \phi_{k-1}^i(\mathbf{y}_{k-1}) \phi_{k}^j(\mathbf{y}_{k}) \Phi_{k}(\mathbf{z}_{k-1}, \mathbf{z}_{k}) d\mathbf{y}_{k-1} d\mathbf{y}_{k}\,. \label{eq: Precompute_formula}
	\end{equation}
	Similarly, if $\rightmesskminus = \sum_{i=1}^{\infty} r_{k-1}^{i} \otimes \phi_{k-1}^{i}$, then the coefficients of $\rightmessk = \rightkminusop(\rightmesskminus, \upmesskminus)$ in the basis $(\phi_{k}^i)_{i=1}^\infty$ are given by
	\begin{equation}
		r_{k}^i(x_{k}) = \sum_{x_{k-1} \in \cX_{k-1}} \upmesskminus(x_{k-1}) \sum_{j=1}^\infty r_{k-1}^j(x_{k-1}) 	\Gamma^{ij}_{k-1}(x_{k-1}, x_{k})\,.
	\end{equation}
\end{lemma}


To obtain a practical procedure, we replace the infinite sums in \eqref{approx: left}-\eqref{approx: right} with finite approximations.
Choosing a sufficiently large $M$, and using the first $M$ orthonormal functions on the basis to approximate $\leftmessk$ and $\rightmessk$, we repeat the previous steps to derive the update rules, expressed as matrix-vector multiplications.
\begin{gather}
	    \upmessk(x_k) \leftarrow \mu(x_k) (\mathbf{\bl}_{k}(x_k)^T \mathbf{r}_{k}(x_k))^{-1}, \label{VecUpdate: c_k}\\
    \bl_{k-1}(x_{k-1}) {\leftarrow} \sum_{x_{k} \in \cX_k} \upmessk(x_k) \mathbf{\Gamma}_{k-1}(x_{k-1}, x_{k}) \bl_{k}(x_{k}) \label{VecUpdate: left_coef} \\
    \br_{k}(x_{k}) {\leftarrow}  \sum_{x_{k-1} \in \cX_{k-1}} \upmesskminus(x_{k-1}) \br^T_{k-1}(x_{k-1}) \mathbf{\Gamma}_{k-1}(x_{k-1}, x_{k})
     \label{VecUpdate: right_coef}
\end{gather}
where $\bl_{k-1}(x_{k-1})$ and $\br_{k}(x_{k})$ are vectors in $\mathbb{R}^M$ and $\mathbf{\Gamma}_{k-1}(x_{k-1}, x_{k})$ is a matrix in $\mathbb{R}^{M \times M}$ whose element in row $i$ and column $j$ is given by $\Gamma_{k-1}^{ij}(x_{k-1}, x_{k})$. 

\begin{algorithm} \label{alg: final_message_passing}
\caption{Approximate Belief Propagation Algorithm}
\begin{algorithmic} \label{algo: base_approx_mp}
\STATE Precompute $\mathbf{\Gamma}_0, ..., \mathbf{\Gamma}_{K-1} \in \mathbb{R}^{n \times n \times M \times M}$ by \eqref{eq: Precompute_formula}. 
\STATE Initialize $\{ \mathbf{r}_k(x_k) \}_{k, x_k}$ and $\{ \mathbf{l}_k(x_k) \}_{k, x_k}$ as $M$ dimensional vectors filled with 1's
\WHILE{\text{~not converged~}}

\FOR{$k=K,...,1$}
%    \FOR{ $x_{k} \in \mathcal{X}_{k}$}
%    \STATE Calculate $\upmessk(x_k)$ by \eqref{VecUpdate: c_k}
%    \ENDFOR
%    \FOR{$x_{k-1} \in \mathcal{X}_{k-1}$}
    \STATE  \text{Update $\bl_{k-1}$ by \eqref{VecUpdate: left_coef}} 
%    \ENDFOR
\ENDFOR

%\FOR{$x_{0} \in \mathcal{X}_{0}$}
    \STATE Calculate $\upmesszero$ by \eqref{VecUpdate: c_k}
%\ENDFOR

\FOR{$k=1,...,K$}
%    \FOR{$x_{k} \in \mathcal{X}_{k}$}
\STATE  \text{Update $\br_{k}$ by \eqref{VecUpdate: right_coef}} 
    \STATE Calculate $\upmessk$ by \eqref{VecUpdate: c_k}
%    \ENDFOR
\ENDFOR

\ENDWHILE
\STATE Return $\br_k$ and $\bl_k$
\end{algorithmic}
\end{algorithm}

Upon convergence of this algorithm, we obtain the coefficients $\br_{k}$ and $\bl_k$, and thereby obtain estimates of $\upmessk^*$.
As discussed after \cref{thm: poly_time_epsilon_approx}, these messages can be used directly for downstream tasks involving the Schrödinger bridge.
%Since $\upmessk$ possesses an explicit formula in terms of these coefficients, the output of Algorithm~\ref{algo: base_approx_mp} 
% The following algorithm illustrates how to use these coefficients to recover $p_{\alpha_{k, k+1}}(\mathbf{z}_k, \mathbf{z}_{k+1})$ and sample trajectories based on observations. 

\section{Time complexity and practical considerations}\label{sec:practical}
Implementing Algorithm~\ref{algo: base_approx_mp} requires selecting bases $(\{\phi_k^i\}_{i=1}^\infty)_{k \in [K]}$ along with a number of coefficients $M$.
The computational complexity of the resulting algorithm scales directly with $M$, which we summarize in the following result.
\begin{theorem}
	Executing $T$ iterations of \cref{algo: base_approx_mp} takes $O(T Kn^2 M^2)$ time.
	In particular, executing $T = \tilde O(K C_{\max} \epsilon^{-1})$ iterations takes $\tilde O(K^2 n^2 M^2 C_{\max} \epsilon^{-1})$ time. 
\end{theorem}
\begin{proof}
For each iteration of Algorithm~\ref{algo: base_approx_mp}, we run $2K$ sub-iterations for updating the left and right messages $\bl_k$ and $\br_k$. The intermediate step~\eqref{VecUpdate: c_k} for the calculation of $\upmessk$ has complexity $O(nM)$. The major update steps~\eqref{VecUpdate: left_coef} and~\eqref{VecUpdate: right_coef} involve matrix-vector multiplication with a matrix of size~$nM \times nM$ , which has complexity $O(n^2M^2)$. Therefore, the total complexity of the algorithm is given by~$O(T Kn^2 M^2)$.
\end{proof}
\Cref{thm: poly_time_epsilon_approx} suggests that $T = \tilde O(K C_{\max} \epsilon^{-1})$ iterations suffice to obtain a $\epsilon$-approximate solution to~\eqref{eq:lifted_eot}; unfortunately, however, we lack a rigorous approximation guarantee quantifying the difference between the output of \cref{algo: base_approx_mp} and that of \cref{alg: BP-continuous}.
Nevertheless, the success of our empirical results (\cref{sec:experiments}) indicates that \cref{algo: base_approx_mp} does offer a good approximation for the solution to the smooth SB problem.
We leave the open question of demonstrating this fact theoretically to future work.

The main tuning parameter of our algorithm is the choice of $M$.
In principle, this choice should depend on the smoothness of the messages $\leftmessk$ and $\rightmessk$, the order $m$ of the GAP, and the dimension $d$.
Since $\leftmessk$ and $\rightmessk$ correspond to Gaussian densities, their expansion in many reasonable bases (for example, Fourier or Wavelet bases) will exhibit strong decay; however, since they are defined on $\cY_k = \bR^{(m-1)d}$, standard smoothness arguments would predict that the necessary number of coefficients scales exponentially with the product $md$.

However, the dependence on $d$ can be somewhat ameliorated under additional assumptions.
Suppose that the GAP has independent coordinates and the orthogonal bases have tensor product structure, so that each basis element $\phi \in L^2(\bR^{(m-1)d})$ satisfies $\phi(\by) = \prod_{j=1}^d \varphi^{(j)}(\by^{(j)})$
for $\varphi^{(j)} \in L^2(\bR^{m-1})$ and where $\by^{(j)}$ corresponds to the derivatives of the $j$th coordinate of $\omega$.
In this case, the tensor $\boldsymbol{\Gamma}$ factors across each dimension into the tensor product of $d$ smaller tensors $\tilde{\Gamma}^{(j)}$,$(j=1,...,d)$. Suppose the number of coefficients we use is equal for each dimension, i.e. $\tilde{\Gamma}^{(j)} \in \mathbb{R}^{n \times n \times M^{\frac{1}{d}} \times M^{\frac{1}{d}}}$, then the complexity of steps~\eqref{VecUpdate: left_coef} and~\eqref{VecUpdate: right_coef} drops to $O(dn^2M^{1+\frac{1}{d}})$ by taking advantage of this lower rank structure.  In this important special case, therefore, the time complexity of our algorithm scales more benignly with $d$, which allows us to take larger $M$ when $d$ rises. A record of the running time of one iteration of message passing against $M $ and dimension $d$ is presented in Table~\ref{tb:runtime}.
\section{Experiments}~\label{sec:experiments}
\noindent We test our algorithm on two kinds of smooth trajectory inference tasks. The first kind aims at tracking the exact trajectory of each individual particle (e.g. Figure~\ref{FIG:Matern_1D}), which we refer to as the One-By-One (OBO) tracking task in the following text. For this kind of task, we evaluate the performance by calculating the distance of each inferred trajectory and the ground truth and measure the percentage of time that the algorithm tracks a particle correctly. For the second kind, the task is to infer the group trajectories of point clouds whose evolution has geometric structures. We provide two ways to evaluate the performance for this kind of task, similar to the evaluation in~\cite{banerjee2024efficient}. We first keep all the observations and visualize the trajectories and see if they form a pattern that is close to the ground-truth pattern. Secondly, we will leave out observations at a certain timestep and instead infer the position of particles at this timestep and evaluate the distance between the inferred and real observations, which we call Leave-One-Timestep-Out (LOT) tasks. Our code for reproducing these experiments is available on~\href{https://github.com/WanliHongC/Smooth_SB}{Github}.
\subsection{One-By-One tracking}
For OBO tasks, we consider three synthetic datasets where trajectories of particles intersect frequently. We compare our algorithm with the standard Schrödinger Bridge (SB) and a modification based on computing the $W_2$ optimal matching at each step (W2M). We test on three data sets, two 2-dimensional data sets (Fig~\ref{FIG:trima} in \cref{sec:details}) and a 3-dimensional data set consisting of the simulated orbits of an $N$-body physical system (Fig.~\ref{FIG:nbody_f1}). Smooth SB performs second-best on the Tri-stable diffusion dataset and substantially outperforms other approaches on the more challenging $N$-Body and Gaussian Process data. Quantitative evaluations are summarized in Table~\ref{tab:obo_quan}. Full experimental details appear in~\cref{sec:details}.


\begin{figure}[t] 

	\centering
	\includegraphics[scale=0.5]{../Figures/icml_nbody.png}
	
	\caption{Visualization of orbits in 3D space. The colors of trajectories depend on the starting point. The second row is the visualization of the XY-space projection of the corresponding above plot.}
    \label{FIG:nbody_f1}
    \vspace{-3pt}
\end{figure}

\begin{table}
\centering
\caption{A comparison between smooth SB and two baseline particle tracking methods. %Smooth SB performs second-best on the Tri-stable diffusion dataset and substantially outperforms other approaches on the more challenging N Body and Gaussian Process data.
	Information on evaluation metrics appears in \cref{sec:details}.}
\label{tab:obo_quan}
\begin{tabular}{l|l|r|r|r}
\toprule
Dataset & Method &  $\mathrm{JumpP} (\downarrow)$& $\mathrm{5p~acc} (\uparrow)$& $\mathrm{Mean} ~ \ell_2 (\downarrow)$\\
\midrule
% 1D Smooth& LSB (ours)& \textbf{4.76e-2}& \textbf{0.893}& \textbf{2.55e-3}\\
%   Gaussian& BMSB& & & \\
%  Process& W2M& 2.18e-1& 0.412& 1.53e-1\\
% \midrule
Tri-stable& SSB (ours)& 1.12e-1& 0.798& 1.42e-2\\
 Diffusion& BMSB& 5.20e-1& 0.171& 6.79e-1\\
 & W2M& \textbf{2.25e-2}& \textbf{0.956}& \textbf{1.37e-8}\\
 \midrule
 N Body& SSB (ours)& \textbf{5.00e-4}& \textbf{0.999}& \textbf{5.48e-4}\\
 & BMSB& 1.14e-1& 0.641& 5.43e-1\\
 & W2M& 1.08e-1& 0.649& 5.50e-1\\
  \midrule
 2D & SSB (ours)& \textbf{5.60e-3}& \textbf{0.991}&\textbf{3.57e-4}\\
 Gaussian & BMSB& 1.37e-1& 0.612&2.82e-1\\
 Process& W2M& 6.60e-2& 0.760&2.32e-1\\
\end{tabular}
\end{table}

\subsection{Point clouds trajectory inference}
We also test our algorithm on four challenging baselines in the trajectory inference literature. We compare our algorithm quantitatively on tasks of LOT with three other state-of-the-art algorithms: MIOFlow~\cite{huguet2022manifold}, DMSB~\cite{CheLiuTao23} and F\&S~\cite{pmlr-v130-chewi21a}. A visualization of the output of our algorithm appears in~Figure~\ref{FIG:visual_all} and the quantitative results for the LOT tasks are provided in Table~\ref{tab:lot2}. The full experimental details appear in~\cref{sec:details}.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{../Figures/icml_visual_lsb.png}
	
	\caption{Visualization of trajectory inference on various datasets by lifted SB, for the $5$D Dyngen Tree data, we visualize the 2D projection of the first three dimensions in the second row.}
    \label{FIG:visual_all}
\end{figure}


\begin{table}[h!]
\centering
\caption{Performance comparison on the Leave-One-Timestep-Out task at step $j$ between our algorithm and the state-of-art algorithms.
Our algorithm is typically \textbf{best} or \textit{second-best}.  DMSB failed to converge on the Dyg dataset despite extensive tuning.  Information on evaluation metrics appears in \cref{sec:details}.}
\label{tab:lot2}
\begin{tabular}{l|l|r|r|r}
\toprule
Dataset & Method &  $\mathbf{W}_1 (\downarrow)$& $\mathbf{M}_G (\downarrow)$& $\mathbf{M}_I (\downarrow)$\\
\midrule
Petal& SSB (ours)& \textit{2.70e-2}& \textbf{2.21e-5}& \textbf{3.75e-3}\\
 $j = 2$&  MIOFlow& 2.22e-1& 9.06e-3& 1.11e-1\\
 & DMSB& 2.10e-1& 5.52e-3& 3.68e-2\\
 & F\&S& \textbf{2.05e-2}& \textit{2.85e-5}&\textit{4.48e-3}\\
\midrule
 EB& SSB (ours)& \textbf{8.45e-2}& 2.46e-3& 5.04e-2\\
 $j = 2$&  MIOFlow& 1.34e-1& \textbf{1.36e-3}& \textbf{2.81e-2}\\
 & DMSB& 1.46e-1& 9.43e-3& 9.72e-2\\
 & F\&S& \textit{8.72e-2}& \textit{1.47e-3}&\textit{3.88e-2}\\
\midrule
Dyg& SSB (ours)& \textit{9.81e-2}& \textbf{1.64e-3}& \textbf{3.51e-2}\\
 $j = 1$& MIOFlow 
& 2.33e-1& 2.82e-2& 1.73e-1\\
 & DMSB
& *& *&* \\
 & F\&S& \textbf{9.78e-2}& \textit{2.00e-3}& \textit{4.64e-2}\\
\end{tabular}
\end{table}
\section{Discussions and Future Directions}
We have presented a new method for trajectory inference and particle tracking based on smooth Schrödinger bridges, which achieves very good performance on a number of challenging benchmarks.
The main limitations of our proposal are related to the approximate implementation developed in Section~\ref{sec:approx_bp}.
As we have discussed, our proposal suffers from the curse of dimensionality, because the number of coefficients $M$ typically scales exponentially with respect to both the order of the GAP ($m$) and the dimension of the observations ($d$).
In numerical experiments, relatively small values of $M$ (of order 1000) seem to perform well for problems up to dimension 5.
An important question for future work is to either develop an approach with better dimensional scaling or, alternatively, show that the exponential scaling in dimension is unavoidable, as is the case for Wasserstein barycenters~\cite{AltBoi22}.

Implementing our approach also requires selecting a suitable GAP to use as a reference process.
As our experiments make clear, it is not necessary that the reference process match the data generating process precisely (see, e.g., Figure~\ref{FIG:Matern_1D}).
However, picking an appropriate variance for the Gaussian process is important for good performance (see Figure~\ref{FIG:c_compare}).
In our experiments, choosing $\sigma \approx \sigma_{\mathrm{data}}$ where $\sigma_{data} \in \mathbb{R}^d$, the empirical variance of the observations along each dimension, typically works well.

Finally, we have considered a definition of the Schrödinger bridge which enforces the strict marginal constraint $P_k = \mu_k$.
In applications, it is natural to assume that observations of the particles are corrupted with noise, which motivates a version of the SB with an approximate constraint $P_k \approx \mu_k$~\cite{ChiZhaHei22,LavZhaKim24}.
It is possible to incorporate noisy observations into the graphical model framework we describe above by introducing a suitable potential at the factor nodes $\alpha_k$.
We leave this extension to future work.

\section*{Acknowledgments}
JNW acknowledges the support of NSF grant DMS-2339829.



% \begin{tabular}{| p{3cm}|p{3cm}|p{3cm}  |l}
% \hline
% \multicolumn{4}{c}{Country List}\\
% \hline
% Dataset &Methods &Hold Out Timestep & $\BW$_1 & MMD1 & MMD2\\
% \hline
% Petal& LSB &0.059866&0.000632&\\
% MIO& AX   & ALA  &\\
% FSI&AL & ALB  &\\
% Algeria    &DZ & DZA  &\\
% American Samoa & AS & ASM  &\\
% Andorra & AD & AND    &\\
% Angola & AO & AGO  &\\
% \hline
% \end{tabular}
